Low-Rank Approximation of Weighted Tree Automata

We describe a technique to minimize weighted tree automata (WTA), a powerful formalisms that subsumes probabilistic context-free grammars (PCFGs) and latent-variable PCFGs. Our method relies on a singular value decomposition of the underlying Hankel matrix defined by the WTA. Our main theoretical result is an efficient algorithm for computing the SVD of an infinite Hankel matrix implicitly represented as a WTA. We provide an analysis of the approximation error induced by the minimization, and we evaluate our method on real-world data originating in newswire treebank. We show that the model achieves lower perplexity than previous methods for PCFG minimization, and also is much more stable due to the absence of local optima.

==> svta_bound.tex <==
\section{New attempt at the bound}

%
%
%
%
%
%
%
%
%
%
%
To prove Theorem~\ref{thm:svtabound}, we will show how the computation of a
WTA on a give tree $t$ can be seen as an inner product between two tensors, one
which is a function of the topology of the tree, and one which is a function of the
labeling of its leafs (Proposition~\ref{prop:innerproduct_topo_leafs}). We will then 
show a fundamental relation between the components of the first tensor and the 
singular values of the Hankel matrix when the WTA is in SVTA normal form 
(Proposition~\ref{prop:singv_and_multicontexts}); this proposition will allow us
to show Lemma~\ref{lemma:multicontext_SVTA_truncation_bound} that bounds
the difference between components of this first tensor for the original SVTA and
its truncation. We will finally use this lemma to bound the absolute error introduced
by the truncation of an SVTA (Propositions~\ref{prop:bound_tree} and~\ref{prop:bound_sumtree}).

We first introduce another kind of contexts than the one introduced in Section~\ref{sec:approxmin},
where every leaf of a binary tree is labeled by the special symbol $*$ (which still acts
as a place holder). 
Let $\Bs$ be the set of binary trees on the one-letter alphabet $\{*\}$. 
We will call a tree $b\in \Bs$ a \emph{multicontext}. 
For any integer $M\geq 1$ we let 
$$\Bs_M =\{ b\in \Bs : |\yield{b}| = M\}$$
be the subset of multicontexts with $M$ leaves (equivalently, $\Bs_M$ is the subset
of multicontexts of size $M-1$).
%
Given a word $w = w_1\cdots w_M \in \Sigma^*$ and a multicontext $b\in \Bs_{M}$, 
we denote by $b[w_1,\cdots,w_M] \in \Ts_\Sigma$ the tree obtained by replacing the
$i$th occurrence of  $*$ in $b$ by $w_i$ for $i\in [M]$.
%
Let $b\in \Bs_M$, for any integer $m \in [M]$ we denote by 
$b\llbracket m \rrbracket\in \Bs_{M+1}$ the multicontext obtained
by replacing the $m$th occurence of $*$ in $b$ by the tree $(*,*)$.
Let $M>1$, it is easy to check that for  any $b'\in \Bs_M$, there
exist $b \in \Bs_{M-1}$ and $m \in [M-1]$ satisfying $b' = b\llbracket m \rrbracket$. 
See Figure~\ref{fig:multicontexts} for some illustrative examples.

\begin{figure}
\begin{center}
\includegraphics[scale=1]{./figures/multicontexts.pdf}
\end{center}
\caption{A multicontext $b = ((*,*),*) \in\Bs_3$, the tree $b[e,g,f] \in \Ts$ and the
multicontext $b\llbracket 2 \rrbracket \in \Bs_4$. }
\label{fig:multicontexts}
\end{figure}


We now show how the computation of a WTA on a given tree with $M$ leaves can be
seen as an inner product between two $M$th order tensors: the first one depends
on the topology of the tree, while the second one depends on the labeling of its
leaves. Let $A = \wtaSigma$ be a WTA with $n$ states computing a function $f$. 
Given a multicontext 
$b\in \Bs_M$, we denote by $\wzeroB_A(b) \in \bigotimes_{i=1}^M \R^n$ the
$M$th order tensor inductively defined by $\wzeroB_A(*) = \wzero$ and
{
\begin{align*}
\MoveEqLeft \wzeroB_A(b\llbracket m \rrbracket)_{i_1 \cdots i_{M}} = 
\sum_{k=1}^n \wzeroB_A(b)_{i_1\cdots i_{m-1} k i_{m+2} \cdots i_{M}}
\T_{k i_{m} i_{m+1}}
\end{align*}
}%
for any $b\in \Bs_{M-1}$, $m\in [M-1]$ and $i_1, \cdots, i_M\in [n]$ 
(i.e. $\wzeroB_A(b\llbracket m \rrbracket)$ is the 
contraction of $\wzeroB_A(b)$ along the $m$th mode and $\T$ along the
first mode).
Given a word $w = w_1\cdots w_M \in \Sigma^*$, we let
$\winfB_A(w) \in \bigotimes_{i=1}^M \R^n$ be the $M$th order tensor defined
by 
{
$$\winfB_A(w)_{i_1\cdots i_M} = \winf(w_1)_{i_1} \winf(w_2)_{i_2}\cdots\winf(w_M)_{i_M}
= \prod_{m=1}^M \winf(w_m)_{i_m}$$
}%
for $i_1,\cdots, i_M \in [n]$ (i.e. $\winfB_A(w)$ is the tensor product of the $\winf(w_i)$'s). 
We will simply write $\wzeroB$ and $\winfB$ when the automaton is clear from context.

\begin{proposition}\label{prop:innerproduct_topo_leafs}
For any multicontext $b\in \Bs_M$ and 
any word $w = w_1\cdots w_M \in \Sigma^* $ we have
$$f(b[w_1,\cdots,w_M]) = \langle \wzeroB(b), \winfB(w) \rangle\enspace,$$
where the inner product between two $M$th order tensors $\ten{U}$ and $\ten{V}$
is defined by $\langle \ten{U},\ten{V}\rangle = \sum_{i_1\cdots i_M} \ten{U}(i_1,\cdots,i_M)\ten{V}(i_1,\cdots,i_M)$.
\end{proposition}
\begin{proof}[Sketch of proof]
Let $b\in \Bs_M$ and  $w = w_1\cdots w_M \in \Sigma^* $. 
Let $b_1 \in \Bs_{M-1}$ and $m\in [M-1]$ be such that
$b = b_1\llbracket m \rrbracket$.
In order to  lighten the notations and without loss of generality we assume that $m =1$.
One can check that
\begin{align*}
 \langle \wzeroB(b), \winfB(w) \rangle  =& \wzeroB(b)(\winf_{w_1}, \cdots, \winf_{w_M})\\
 =& 
 \wzeroB(b_1\llbracket 1 \rrbracket )(\winf_{w_1}, \cdots, \winf_{w_M})\\
 =&
  \wzeroB(b_1)(\winf((w_1,w_2)), \winf_{w_3}, \cdots, \winf_{w_M})\enspace .
\end{align*} 
The same reasoning can now be applied to $b_1$. Assume for example that
$b_1 = b_2 \llbracket 1 \rrbracket$ for some $b_2 \in \Bs_{M-2}$, 
we would have
\begin{align*}
 \langle \wzeroB(b), \winfB(w) \rangle  
 &=
 \wzeroB(b_1)(\winf((w_1,w_2)), \winf_{w_3}, \cdots, \winf_{w_M})\\
 &=
 \wzeroB(b_2\llbracket 1\rrbracket )(\winf((w_1,w_2)), \winf_{w_3}, \cdots, \winf_{w_M}) \\
 &=
 \wzeroB(b_2)(\winf(((w_1,w_2),w_3)), \winf_{w_4}, \cdots, \winf_{w_M})\enspace .
\end{align*}
By applying the same argument again and again we will eventually obtain
\begin{align*}
\langle \wzeroB(b), \winfB(w) \rangle  &=  \wzeroB(b_{M-1})(\winf(b[w_1,\cdots,w_M])) \\
&=  \wzeroB(*)(\winf(b[w_1,\cdots,w_M]))\\
&= \wzero^\top \winf(b[w_1,\cdots,w_M])\\
&= f(b[w_1,\cdots,w_M])\enspace. \qedhere
\end{align*}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


%
%
%
%
%
%
%
\end{proof}


Suppose now that $A = \wtaSigma$ is an SVTA with $n$ states for $f$ and let 
$\singv_1 \geq \singv_2 \geq \cdots \geq \singv_n$ be the singular
values of the Hankel matrix $\mat{H}_f$. 
The following proposition shows a relation --- similar to the one presented in 
Theorem~\ref{prop:singv_and_SVTA_params} --- between the components of
the tensor $\wzeroB(b)$ (for any multicontext $b$) and the singular values of the Hankel matrix.

\begin{proposition}\label{prop:singv_and_multicontexts}
If $A = \wtaSigma$ is an SVTA, then for any $b\in \Bs_M$ and 
any $i_1,\cdots,i_M \in [n]$ the following holds:
$$|\wzeroB(b)_{i_1\cdots i_M}| \leq n^{M-1} \min_{p\in [M]} \{\singv_{i_p} \}
 \prod_{m=1}^M \frac{1}{\sqrt{\singv_{i_m}}} \enspace.$$
 
\end{proposition} 
\begin{proof}
We proceed by induction on $M$. If $M=1$ we have $b=*$ and
$$|\wzeroB(*)_i| = |\wzero_i| \leq \sqrt{\singv_i} = \frac{\singv_i}{\sqrt{\singv_i}}\enspace.$$
Suppose the result holds for multicontexts in $\Bs_{M-1}$ and let
$b'\in \Bs_M$. Let $m \in [M]$ and $b\in \Bs_{M-1}$ be such that 
$b' = b\llbracket m \rrbracket$. Without loss of generality and to lighten
the notations we assume that $m = 1$. Start by writing:
\begin{align*}
|\wzeroB(b')_{i_1\cdots i_M}| = |\wzeroB(b\llbracket 1 \rrbracket)_{i_1 \cdots i_M}| 
&=
\left| \sum_{k=1}^n \wzeroB_A(b)_{ k i_{3} \cdots i_{M}}
\T_{k i_1 i_2} \right| 
\leq
\sum_{k=1}^n \left| \wzeroB_A(b)_{ k i_{3} \cdots i_{M}}
\T_{k i_1 i_2} \right|
\end{align*}
Remarking that the third inequality in Theorem~\ref{prop:singv_and_SVTA_params}
can be rewritten as $|\T_{ijk}| \leq \frac{\min\{\singv_i, \singv_j,
\singv_k\}}{\sqrt{\singv_i}\sqrt{\singv_j}\sqrt{\singv_k}}$, we have for any $k
\in [n]$:
\begin{align*}
\left| \wzeroB_A(b)_{ k i_{3} \cdots i_{M}} \T_{k i_1 i_2} \right| 
\leq&
n^{M-2} \min\{\singv_k,\singv_{i_3},\cdots, \singv_{i_M}\} \frac{1}{\sqrt{\singv_k}} 
\prod_{m=3}^M \frac{1}{\sqrt{\singv_{i_m}}} 
\frac{\min\{\singv_k, \singv_{i_1}, \singv_{i_2}\}}{\sqrt{\singv_k}\sqrt{\singv_{i_1}}\sqrt{\singv_{i_2}}} \\
=&
n^{M-2} \frac{1}{\singv_k}  
\prod_{m=1}^M \frac{1}{\sqrt{\singv_{i_m}}} 
\min\{\singv_k,\singv_{i_3},\cdots, \singv_{i_M}\} \min\{\singv_k, \singv_{i_1}, \singv_{i_2}\}  \\
\leq &
n^{M-2} \min_{p\in [M]} \{\singv_{i_p} \}
 \prod_{m=1}^M \frac{1}{\sqrt{\singv_{i_m}}} \enspace,
\end{align*}
where we used that
$$\min\{\singv_k,\singv_{i_3},\cdots, \singv_{i_M}\} \min\{\singv_k, \singv_{i_1}, \singv_{i_2}\} \leq \singv_k \min\{\singv_{i_1},\cdots, \singv_{i_M}\}$$
Summing over $k$ yields the desired bound.
\qedhere
\end{proof}

Let $\hat{f}$ be the function computed
by the SVTA truncation of $A$ to $\hat{n}$ states. 
Let $\mat{\Pi} \in \R^{n\times n}$ be the diagonal matrix defined by
$\mat{\Pi}(i,i) = 1$ if $i \leq \hat{n}$ and $0$ otherwise. It is easy to 
check that the WTA 
$\hat{A} = \langle\hat{\wzero},\hat{\T},\hat{\winf}_\sigma\rangle$,
where $ \hat{\wzero} =  \mat{\Pi}\wzero$, $\hat{\T}=\T(\I, \mat{\Pi}, \mat{\Pi})$ and
$\hat{\winf}_\sigma =\winf_\sigma$,
computes the function $\hat{f}$. We let $\hat{\winf}(t) = \winf_{\hat{A}}(t)$
for any tree $t$ and similarly for $\hat{\wzero}(c)$, $\hat{\winfB}(w)$ and $\hat{\wzeroB}(c)$.  

We can now prove the following Lemma that bounds the absolute difference
between the components of the tensors $\wzeroB(b)$ and $\hat{\wzeroB}(b)$ for
a given multicontext $b$.

\begin{lemma}\label{lemma:multicontext_SVTA_truncation_bound}
For any $b\in \Bs_M$ and any $i_1,\cdots i_M \in [n]$ we have 
$$|(\wzeroB(b) - \hat{\wzeroB}(b))_{i_1\cdots i_M} | 
\leq \singv_{\hat{n} + 1}\ n^{M-1}  \prod_{m=1}^M \frac{1}{\sqrt{\singv_{i_m}}} \enspace .$$
\end{lemma} 
\begin{proof}
It is easy to check that when there exists at least one $m\in [M]$ such that
$i_m > \hat{n}$, we have $\hat{\wzeroB}(b)_{i_1\cdots i_M} = 0$, 
hence
$$|(\wzeroB(b) - \hat{\wzeroB}(b))_{i_1\cdots i_M} | = |\wzeroB(b)_{i_1\cdots i_M} | $$
and the result directly follows from Proposition~\ref{prop:singv_and_multicontexts}.

Suppose $i_1,\cdots, i_M \in [\hat{n}]$,
we proceed by induction on $M$. If $M=1$ then $b=*$, thus
$$|\wzeroB(*)_i - \hat{\wzeroB}(*)_i| = |\wzero_i - \hat{\wzero}_i| = 0$$
for all $i \in [\hat{n}]$.



Suppose the result holds for multicontexts in $\Bs_{M-1}$ and let
$b' \in \Bs_{M}$. Let $b\in \Bs_{M-1}$ and $m \in [M-1]$ be  such that
$b' = b\llbracket m \rrbracket$. To lighten the notations we assume
without loss of generality that $m = 1$. We have
\begin{align}
|(\wzeroB(b') - \hat{\wzeroB}(b'))_{i_1\cdots i_{M}} | 
\label{eq:multicontext_1}
=&
|(\wzeroB(b\llbracket 1 \rrbracket) - \hat{\wzeroB}(b\llbracket 1 \rrbracket))_{i_1\cdots i_{M}} |\\
\leq&
\label{eq:multicontext_2.1}
\sum_{k=1}^{\hat{n}} \left| \T_{k i_{1} i_2} \right| 
| (\wzeroB(b)  -  \hat{\wzeroB}(b))_{k i_{3}\cdots i_{M}} | \\
+& 
\label{eq:multicontext_2.2}
\hspace{-0.2cm}\sum_{k=\hat{n}+1}^{n} \left| \T_{k i_{1} i_2} \right| \left| \wzeroB(b)_{k i_{3}\cdots i_{M}} \right| \\
\leq &
\label{eq:multicontext_3.1}
\sum_{k=1}^{\hat{n}} \frac{\sqrt{\singv_k}}{\sqrt{\singv_{i_1}\singv_{i_2}}} 
\cdot \frac{\singv_{\hat{n} + 1}\ n^{M-2} }{\sqrt{ \singv_k} \sqrt{\singv_{i_3}} \cdots \sqrt{\singv_{i_M}}} \\
+ & 
\label{eq:multicontext_3.2}
\hspace{-0.2cm}\sum_{k=\hat{n}+1}^{n} \frac{\sqrt{\singv_k}}{\sqrt{\singv_{i_1}\singv_{i_2}}} 
\cdot \frac{\min\{\singv_k, \singv_{i_3}, \cdots, \singv_{i_M}\}\ n^{M-2} }
				 {\sqrt{ \singv_k} \sqrt{\singv_{i_3}} \cdots \sqrt{\singv_{i_M}}} \\
\leq &
\ \singv_{\hat{n}+1}\ n^{M-1}  \prod_{m=1}^{M} \frac{1}{\sqrt{\singv_{i_m}}} \enspace .
\end{align}
To decompose~(\ref{eq:multicontext_1}) in~(\ref{eq:multicontext_2.1}) and~(\ref{eq:multicontext_2.2})
we used the fact that $\T_{k i_1 i_2} = \hat{\T}_{k i_1 i_2}$ whenever $k \leq \hat{n}$ and
$\hat{\wzeroB}(b)_{k i_3\cdots i_M} = 0$ whenever $k > \hat{n}$. We bounded~(\ref{eq:multicontext_2.1}) 
by~(\ref{eq:multicontext_3.1}) using the induction hypothesis, while we used Proposition~\ref{prop:singv_and_multicontexts}
to bound~(\ref{eq:multicontext_2.2}) by~(\ref{eq:multicontext_3.2}).  
\end{proof}


\begin{proposition}\label{prop:bound_tree}
Let $t\in \Ts$ be a tree of size $M$, then 
\begin{align*}
|f(t) - \hat{f}(t)| 
&\leq 
n^{2M-1} \singv_{\hat{n}+1} 
\enspace .
\end{align*}
\end{proposition}
\begin{proof}
Let $t \in \Ts$ be a tree of size $M-1$, then there exists a (unique) $b \in \Bs_{M}$ 
and a (unique) word $w = w_1 \cdots w_{M} \in \Sigma^*$ 
such that $t = b[w_1,\cdots, w_{M} ]$. Since $\winf_\sigma = \hat{\winf}_\sigma$ for
all $\sigma \in \Sigma$, we have $\winfB(x) = \hat{\winfB}(x)$ for all $x\in \Sigma^*$. 
Furthermore, since $\winf_\sigma(i)^2 \leq \singv_i$ for all $i\in [n]$, we have
$$|\winfB(w)_{i_1\cdots i_M}| \leq \prod_{m=1}^M \sqrt{\singv_{i_m}}\enspace.$$  
It follows that 
\begin{align*}
|f(t) - \hat{f}(t)| 
= & 
\left|\langle \wzeroB(b),\winfB(w) \rangle - \langle \hat{\wzeroB}(b),\hat{\winfB}(w) \rangle \right|\\
= &
\left|\langle \wzeroB(b) - \hat{\wzeroB}(b),\winfB(w) \rangle \right|\\
\leq &
\sum_{i_1=1}^n \cdots \sum_{i_M=1}^n |(\wzeroB(b) - \hat{\wzeroB}(b))_{i_1\cdots i_M} |\ | \winfB(w)_{i_1\cdots i_M} |\\
\leq &
\sum_{i_1=1}^n \cdots \sum_{i_M=1}^n \singv_{\hat{n} + 1}\ n^{M-1}  \prod_{m=1}^M \frac{1}{\sqrt{\singv_{i_m}}}
\cdot \prod_{m=1}^M \sqrt{\singv_{i_m}} \\
= &
n^{2M - 1} \singv_{\hat{n} +1}
\end{align*}
\end{proof}

\borja{Here we're not using Holder's inequality but a more basic fact. Would it be possible to exploit the power of Holder in some way by obtaining \emph{aggregate} bounds on the Frobenius norm of the tensors $\wzeroB(b) - \hat{\wzeroB}(b)$?

Another issue is whether we can prove directly that $\hat{f}$ is in some sense bounded, and plug the bound $|f(t)| + |\hat{f}(t)|$ instead of the bound above when $M$ becomes large... The problem with this is that we don't even know how to do this in the string case.}


\begin{proposition}\label{prop:bound_sumtree}
Let $S = |\Sigma|$ be the
size of the alphabet. For any integer $M$ we have
$$ \sum_{t\in\Ts:\atop\size{t} < M}  |f(t) - \hat{f}(t)| \leq  \frac{(4Sn^2)^{M+1}-1}{(4Sn^2)-1} \singv_{\hat{n}+1}\enspace.$$
\end{proposition}
\begin{proof}
For any integer $m$ there are less than $4^m$ binary trees with $m$ internal nodes (which is a bound
on the $m$-th Catalan number) and each one of these trees has $m+1$ leaves, thus $S^{m+1}$ possible
labelling of the leaves. Using the previous proposition we get
\begin{align*}
\sum_{t\in\Ts:\atop\size{t} < M}  |f(t) - \hat{f}(t)| 
 &=
 \sum_{m = 0}^{M-1}   \sum_{t\in\Ts:\atop\size{t} = m}  |f(t) - \hat{f}(t)| \\
&\leq
\sum_{m = 0}^{M-1} 4^m S^{m+1} \cdot  n^{2(m-1)}  \singv_{\hat{n}+1}\\
&\leq
\sum_{m = 1}^{M} (4Sn^2)^{m}  \singv_{\hat{n}+1} \\
&\leq
 \frac{(4Sn^2)^{M+1}-1}{(4Sn^2)-1}  \singv_{\hat{n}+1}.\qedhere
\end{align*}
\end{proof}

\begin{theorem*}
Let $A = \wtaSigma$ be a SVTA with $n$ states realizing a function $f$ and let 
$\singv_1 \geq \singv_2 \geq \cdots \geq \singv_n$ be the singular
values of the Hankel matrix $\mat{H}_f$. Let $\hat{f}$ be the function computed
by the SVTA truncation of $A$ to $\hat{n}$ states.

Let $S=|\Sigma|$ be the size of the alphabet, let $M$ be an integer and let $\varepsilon > 0$.

\begin{itemize}
\item  For any tree $t\in \Ts$ of size $M$,
 if ${\displaystyle M < \frac{\log\left(\frac{1}{\singv_{\hat{n}+1}}\right) + \log\left(\varepsilon\right) }{2\log n} }$
then $|f(t) - \hat{f}(t)| < \varepsilon$.
\item If ${\displaystyle M < \frac{\log\left(\frac{1}{\singv_{\hat{n}+1}}\right) + \log(\varepsilon)}{\log(4Sn^2)} }$ then
$\displaystyle\sum_{t:\size{t}<M} |f(t)-\hat{f}(t)|< \varepsilon$.
\end{itemize}


\end{theorem*}
\begin{proof}
For the first bound, it is easy to check that if 
$$M < \frac{\log\left(\frac{1}{\gamma}\right) + \log\left(\frac{\varepsilon}{4}\right) }{2\log n}$$
then $4 n^{2M} \gamma< \varepsilon$ and the result follows from 
Proposition~\ref{prop:bound_tree}. For the second one, if
$$ M < \frac{\log\left(\frac{1}{\gamma}\right) + \log(\varepsilon)}{2\log(4Sn)} -1$$ then
 $\frac{(4Sn^2)^{M+1}-1}{(4Sn^2)-1}\gamma< \varepsilon$ and the
 result follows from Proposition~\ref{prop:bound_sumtree}.
\end{proof}






\newpage
\clearpage


\section{Old Bound with \textbf{mistake} in the proof!}
Let $A = \wtaSigma$ be a SVTA with $n$ states realizing a function $f$ and let 
$\singv_1 \geq \singv_2 \geq \cdots \geq \singv_n$ be the singular
values of the Hankel matrix $\mat{H}_f$. Let $\hat{f}$ be the function computed
by the SVTA truncation of $A$ to $\hat{n}$ states.

Let $\mat{\Pi} \in \R^{n\times n}$ be the diagonal matrix defined by
$\mat{\Pi}(i,i) = 1$ if $i \leq \hat{n}$ and $0$ otherwise. It is easy to 
check that the WTA 
$\hat{A} = \langle\hat{\wzero},\hat{\T},\hat{\winf}_\sigma\rangle$,
where $ \hat{\wzero} =  \mat{\Pi}\wzero$, $\hat{\T}=\T(\mat{\Pi}, \mat{\Pi}, \mat{\Pi})$ and
$\hat{\winf}_\sigma =\winf_\sigma$,
computes the function $\hat{f}$.

{\color{red} The proof of the following lemma is false!}

\begin{lemma}
Let $c \in \Cs$ be a  context of size $M$. Then
$$| \wzero(c)_j - \hat{\wzero}(c)_j | 
\leq  
\frac{n+\hat{n}}{\sqrt{\singv_j}} \cdot \frac{\hat{n}^{2(M+1)}-1}{\hat{n}^2-1}\sum_{i=\hat{n}+1}^n \singv_i $$
for any $j \in [n]$.
\end{lemma}
\begin{proof}
We proceed by induction on $M$. If $M=0$ then $c=*$, thus
$$|\wzero(*)_j - \hat{\wzero}(*)_j| = |\wzero_j - \hat{\wzero}_j| =
\begin{cases} 
0 &\mbox{ if } j\leq \hat{n} \\
|\wzero_j|&\mbox{ otherwise}
\end{cases} \enspace$$
and for any $j > \hat{n}$ we have
$$ |\wzero_j| \leq \sqrt{\singv_j} \leq \frac{n+\hat{n}}{{\sqrt{\singv_j}}} \sum_{i=\hat{n}+1}^n \singv_i\enspace.$$


Suppose the result holds for contexts of size less than $M$ and let
$c'$ be a context of size $M+1$. Then $c'$ is either of the form
$c' = c[(*,t)]$  or $c' = c[(t,*)]$ for some  $t \in \Ts$ 
and some context $c$ of size less than $M$. Suppose $c' = c[(*,t)]$ (the second
case can be treated analogously), for any $j\in [n]$ we have
\borja{I think the first equation is wrong: shouldn't the term $\hat{\wzero}(c')_j$ be $\T(\mat{\Pi}\hat{\wzero}(c), \mat{\Pi}, \mat{\Pi}\hat{\winf}(t))_j$ (note the hat in $\winf$)?}
{\small
\begin{align*}
\MoveEqLeft
|\wzero(c')_j - \hat{\wzero}(c')_j | = | \T(\wzero(c), \I, \winf(t))_j - \T(\mat{\Pi}\hat{\wzero}(c), \mat{\Pi}, \mat{\Pi}\winf(t))_j|\\
= &
\left| \sum_{i,k=1}^n \T_{ijk}\wzero(c)_i \winf(t)_k  - \sum_{i,k=1}^{\hat{n}} \T_{ijk}\hat{\wzero}(c)_i \winf(t)_k \right|\\
\leq &
\sum_{i,k \in [n] s.t. \atop i>\hat{n}\mbox{ \scriptsize  or } k>\hat{n}} \left| \T_{ijk}\wzero(c)_i \winf(t)_k  \right|\\
&+ 
\sum_{i,k=1}^{\hat{n}} \left| \T_{ijk}(\wzero(c)_i - \hat{\wzero}(c)_i) \winf(t)_k \right|\\
\leq &
\sum_{i=\hat{n}+1}^n \sum_{k=1}^n \frac{\sqrt{\singv_i}}{\sqrt{\singv_j\singv_k}} \sqrt{\singv_i}\sqrt{\singv_k} 
+ \sum_{i=1}^{\hat{n}} \sum_{k=\hat{n}+1}^n \frac{\sqrt{\singv_k}}{\sqrt{\singv_i\singv_j}} \sqrt{\singv_i}\sqrt{\singv_k} \\
&+ 
\sum_{i,k=1}^{\hat{n}} \frac{\sqrt{\singv_i}}{\sqrt{\singv_j\singv_k}} 
  \left(\frac{n+\hat{n}}{\sqrt{\singv_i}} \cdot \frac{\hat{n}^{2M}-1}{\hat{n}^2-1} \sum_{i'=\hat{n}+1}^n \singv_{i'}\right)  
   \sqrt{\singv_k} \\
=&
\frac{ n\displaystyle\sum_{i=\hat{n}+1}^n \singv_i + \hat{n} \displaystyle\sum_{k=\hat{n}+1}^n \singv_k
+
\hat{n}^2 (n+\hat{n}) \frac{\hat{n}^{2M}-1}{\hat{n}^2-1}\displaystyle\sum_{i'=\hat{n}+1}^n \singv_{i'}}{\sqrt{\singv_j}} \\
\leq&
\frac{n+\hat{n}}{\sqrt{\singv_j}} \cdot \frac{\hat{n}^{2(M+1)}-1}{\hat{n}^2-1}\sum_{i=\hat{n}+1}^n \singv_{i} 
\end{align*}
}%
where we used 
$|\T_{ijk}|^2 \leq \min\left\{\frac{\singv_i}{\singv_j\singv_k},
\frac{\singv_j}{\singv_i\singv_k},\frac{\singv_k}{\singv_i\singv_j}\right\}$,
$|\wzero(c)_i| \leq \sqrt{\singv_i}$ and
$|\winf(t)_i| \leq \sqrt{\singv_i}$
for all $i,j,k\in[n]$, $c\in\Cs$ and $t\in \Ts$.

\end{proof}



\begin{proposition}\label{prop:bound_tree}
Let $t\in \Ts$ be a tree of size $M$, then 
\begin{align*}
|f(t) - \hat{f}(t)| 
%
%
&\leq 
4 n^{2(M+1)} \sum_{i=\hat{n}+1}^n \singv_i
\enspace .
\end{align*}
%
%
%
%
%
%
%
%
%
%
%
%

\end{proposition}
\begin{proof}
Let $t$ be a tree of size $M$, then there exists a context $c\in\Cs$ of size $M$ and some $\sigma\in\Sigma$ 
such that $t = c[\sigma]$. Using the previous Lemma, we have
\begin{align*}
\MoveEqLeft
|f(t) - \hat{f}(t)| = | \wzero(c)^\top\winf_\sigma - \hat{\wzero}(c)^\top\hat{\winf}_\sigma|\\
&=
| ( \wzero(c) - \hat{\wzero}(c) )^\top  \winf_\sigma |\\
&\leq \sum_{j=1}^n |\wzero(c)_j - \hat{\wzero}(c)_j | \ |(\winf_\sigma)_j|\\
&\leq 
\sum_{j=1}^n \left(\frac{n+\hat{n}}{\sqrt{\singv_j}} \cdot 
\frac{\hat{n}^{2(M+1)}-1}{\hat{n}^2-1}\sum_{i=\hat{n}+1}^n \singv_i\right) \sqrt{\singv_j}\\
&\leq 
n(n+\hat{n})  \frac{\hat{n}^{2(M+1)}-1}{\hat{n}^2-1}\sum_{i=\hat{n}+1}^n \singv_i\\
&\leq 
2 (n^{2(M+1)} - 1) \frac{n^2}{n^2-1}\sum_{i=\hat{n}+1}^n \singv_i\\
&\leq 4 n^{2(M+1)} \sum_{i=\hat{n}+1}^n \singv_i
\enspace .\qedhere
\end{align*}
\end{proof}

\begin{proposition}\label{prop:bound_sumtree}
Let $S = |\Sigma|$ be the
size of the alphabet. For any integer $M$ we have
$$ \sum_{t\in\Ts:\atop\size{t} < M}  |f(t) - \hat{f}(t)| \leq  \frac{(4Sn^2)^{M+1}-1}{(4Sn^2)-1} \sum_{i=\hat{n}+1}^n \singv_i\enspace.$$
\end{proposition}
\begin{proof}
For any integer $m$ there are less than $4^m$ binary trees with $m$ internal nodes (which is a bound
on the $m$-th Catalan number) and each one of these trees has $m+1$ leaves, thus $S^{m+1}$ possible
labelling of the leaves. Using the previous proposition we get
\begin{align*}
\MoveEqLeft
\sum_{t\in\Ts:\atop\size{t} < M}  |f(t) - \hat{f}(t)| 
 =
 \sum_{m = 0}^{M-1}   \sum_{t\in\Ts:\atop\size{t} = m}  |f(t) - \hat{f}(t)| \\
&\leq
\sum_{m = 0}^{M-1} 4^m S^{m+1} \cdot 4 n^{2(m+1)}  \sum_{i=\hat{n}+1}^n \singv_i\\
&=
\sum_{m = 1}^{M} (4Sn^2)^{m} \sum_{i=\hat{n}+1}^n \singv_i\\
&\leq
 \frac{(4Sn^2)^{M+1}-1}{(4Sn^2)-1} \sum_{i=\hat{n}+1}^n \singv_i\enspace.\qedhere
\end{align*}
\end{proof}

\begin{theorem}
Let $A = \wtaSigma$ be a SVTA with $n$ states realizing a function $f$ and let 
$\singv_1 \geq \singv_2 \geq \cdots \geq \singv_n$ be the singular
values of the Hankel matrix $\mat{H}_f$. Let $\hat{f}$ be the function computed
by the SVTA truncation of $A$ to $\hat{n}$ states.

Let $S=|\Sigma|$ be the size of the alphabet, let 
$\gamma = \singv_{\hat{n}+1} + \cdots + \singv_{n}$,
and let $\varepsilon > 0$.

\begin{itemize}
\item  For any tree $t\in \Ts$ of size strictly less than $M$,
$$\text{if }M < \frac{\log\left(\frac{1}{\gamma}\right) + \log\left(\frac{\varepsilon}{4}\right) }{2\log n} 
\text{ then }|f(t) - \hat{f}(t)| < \varepsilon\enspace.$$
\item For any integer $M$,
if ${\displaystyle M < \frac{\log\left(\frac{1}{\gamma}\right) + \log(\varepsilon)}{2\log(4Sn)} -1}$ then
$$\sum_{t:\size{t}<M} |f(t)-\hat{f}(t)|< \varepsilon\enspace.$$
\end{itemize}


\end{theorem}
\begin{proof}
For the first bound, it is easy to check that if 
$$M < \frac{\log\left(\frac{1}{\gamma}\right) + \log\left(\frac{\varepsilon}{4}\right) }{2\log n}$$
then $4 n^{2M} \gamma< \varepsilon$ and the result follow from 
Proposition~\ref{prop:bound_tree}. For the second one, if
$$ M < \frac{\log\left(\frac{1}{\gamma}\right) + \log(\varepsilon)}{2\log(4Sn)} -1$$ then
 $\frac{(4Sn^2)^{M+1}-1}{(4Sn^2)-1}\gamma< \varepsilon$ and the
 result follow from Proposition~\ref{prop:bound_sumtree}.
\end{proof}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%






%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
















%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


